MIPGAN -- Generating Strong and High Quality Morphing Attacks Using Identity Prior Driven GAN

Face morphing attacks target to circumvent Face Recognition Systems (FRS) by employing face images derived from multiple data subjects (e.g., accomplices and malicious actors). Morphed images can be verified against contributing data subjects with a reasonable success rate, given they have a high degree of facial resemblance. The success of morphing attacks is directly dependent on the quality of the generated morph images. We present a new approach for generating strong attacks extending our earlier framework for generating face morphs. We present a new approach using an Identity Prior Driven Generative Adversarial Network, which we refer to as MIPGAN (Morphing through Identity Prior driven GAN). The proposed MIPGAN is derived from the StyleGAN with a newly formulated loss function exploiting perceptual quality and identity factor to generate a high quality morphed facial image with minimal artefacts and with high resolution. We demonstrate the proposed approach's applicability to generate strong morphing attacks by evaluating its vulnerability against both commercial and deep learning based Face Recognition System (FRS) and demonstrate the success rate of attacks. Extensive experiments are carried out to assess the FRS's vulnerability against the proposed morphed face generation technique on three types of data such as digital images, re-digitized (printed and scanned) images, and compressed images after re-digitization from newly generated MIPGAN Face Morph Dataset. The obtained results demonstrate that the proposed approach of morph generation poses a high threat to FRS.

==> Tables.tex <==

%% Vulnerability (MMPMR and FMMPMR) - Ablation study

\begin{table}[htbp]
  \centering
  \caption{Vulnerability - Ablation study}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|p{5.765em}|p{5.435em}|p{5.335em}|p{6.9em}|r|r|r|r|}
    \hline
    \multirow{2}[4]{*}{\textbf{Final ID}} & \multirow{2}[4]{*}{\textbf{Identity loss}} & \multirow{2}[4]{*}{\textbf{MSSIM}} & \multirow{2}[4]{*}{\textbf{Perceptual}} & \multicolumn{2}{p{11.2em}|}{\textbf{MIPGAN-I}} & \multicolumn{2}{p{12.77em}|}{\textbf{MIPGAN-II}} \bigstrut\\
\cline{5-8}    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{5.535em}|}{FMMPMR} & \multicolumn{1}{p{5.665em}|}{MMPMR} & \multicolumn{1}{p{5.635em}|}{FMMPMR} & \multicolumn{1}{p{7.135em}|}{MMPMR} \bigstrut\\
    \hline
    Final ID & -     & -     & -     & 81.82 & 90.69 & 77.83 & 90.12 \bigstrut\\
    \hline
    -     & Identity loss & -     & -     & 78.15 & 89.17 & 78.39 & 90.04 \bigstrut\\
    \hline
    -     & -     & MSSIM & -     & 80.82 & 91.81 & 78.73 & 89.58 \bigstrut\\
    \hline
    -     & -     & -     & Perceptual & 21.37 & 44.18 & 11.92 & 29.47 \bigstrut\\
    \hline
    -     & -     & -     & -     & \textbf{84.65} & \textbf{94.36} & \textbf{81.59} & \textbf{92.93} \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:vulnerability}%
\end{table}%



%%%%%%%%%%% MAD tables %%%%%%%%

%%%% MAD - Landmarks %%%%%%%%
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{MAD Facial Landmark}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|p{8.665em}|r|r|r|r|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[6]{*}{Morph Generation Type}} & \multirow{3}[6]{*}{MAD Algorithms} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-EER (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER =} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-ERR (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER=} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-EER (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER=} \bigstrut\\
\cline{4-5}\cline{7-8}\cline{10-11}          & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c|}{5\%} & \multicolumn{1}{c|}{10\%} &       & \multicolumn{1}{c|}{5\%} & \multicolumn{1}{c|}{10\%} &       & \multicolumn{1}{c|}{5\%} & \multicolumn{1}{c|}{10\%} \bigstrut\\
\cline{3-11}          & \multicolumn{1}{c|}{} & \multicolumn{3}{p{12.705em}|}{Digital} & \multicolumn{3}{p{12.705em}|}{Print-Scan} & \multicolumn{3}{p{12.705em}|}{Print-Scan with Compression} \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Facial Landmarks}} & Ensemble Features & 0     & 0     & 0     & 1.85  & 0.85  & 0.34  & 2.25  & 1.12  & 0.51 \bigstrut\\
\cline{2-11}          & Hybrid Features & 0.16  & 0     & 0     & 2.35  & 1.45  & 0.96  & 2.58  & 1.71  & 1.54 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 0.22  & 0     & 0     & 1.69  & 0.85  & 0.34  & 14.77 & 27.27 & 19.38 \bigstrut\\
\cline{2-11}          & Hybrid Features & 0.16  & 0     & 0     &       &       &       & 9.44  & 14.57 & 9.14 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 39.16 & 73.14 & 65.35 & 9.45  & 14.57 & 8.74  & 8.95  & 15.26 & 9.26 \bigstrut\\
\cline{2-11}          & Hybrid Features & 46.82 & 86.62 & 81.64 & 12.32 & 19.72 & 13.2  & 9.74  & 15.95 & 8.91 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 34.13 & 70.49 & 61.57 & 5.32  & 6.68  & 2.57  & 6.72  & 8.16  & 4.14 \bigstrut\\
\cline{2-11}          & Hybrid Features & 44.96 & 83.7  & 75.47 & 5.9   & 8.42  & 3.23  & 5.67  & 6.18  & 2.91 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADLandmark}%
\end{table}%



%%%% MAD - StyleGAN %%%%%%%%
\begin{table}[htbp]
  \centering
  \caption{MAD - StyleGAN}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|p{9.065em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{\textbf{D-EER (\%)}}} & \multicolumn{2}{p{8.47em}|}{\textbf{BPCER@APCER =}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{\textbf{D-ERR (\%)}}} & \multicolumn{2}{p{8.47em}|}{\textbf{BPCER@APCER=}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{\textbf{D-EER (\%)}}} & \multicolumn{2}{p{8.47em}|}{\textbf{BPCER@APCER=}} \bigstrut\\
\cline{4-5}\cline{7-8}\cline{10-11}          & \multicolumn{1}{c|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
\cline{3-11}          & \multicolumn{1}{c|}{} & \multicolumn{3}{p{12.705em}|}{Digital} & \multicolumn{3}{p{12.705em}|}{Print-Scan} & \multicolumn{3}{p{12.705em}|}{Print-Scan with Compression} \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[4]{*}{Facial Landmarks}} & \multirow{2}[2]{*}{Ensemble Features} & \multirow{2}[2]{*}{0.32} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{16.16} & \multirow{2}[2]{*}{28.13} & \multirow{2}[2]{*}{19.89} & \multirow{2}[2]{*}{13.89} & \multirow{2}[2]{*}{22.12} & \multirow{2}[2]{*}{17.66} \bigstrut[t]\\
          & \multicolumn{1}{r|}{} &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-11}          & Hybrid Features & 0.42  & 0     & 0     & 15.26 & 26.41 & 17.66 & 14.37 & 22.81 & 16.92 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[4]{*}{StyleGAN}} & \multirow{2}[2]{*}{Ensemble Features} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} & \multirow{2}[2]{*}{0} \bigstrut[t]\\
          & \multicolumn{1}{r|}{} &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-11}          & Hybrid Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[4]{*}{MIPGAN-I}} & \multirow{2}[2]{*}{Ensemble Features} & \multirow{2}[2]{*}{39.97} & \multirow{2}[2]{*}{75.98} & \multirow{2}[2]{*}{68.78} & \multirow{2}[2]{*}{20.21} & \multirow{2}[2]{*}{42.14} & \multirow{2}[2]{*}{33.44} & \multirow{2}[2]{*}{20.73} & \multirow{2}[2]{*}{45.28} & \multirow{2}[2]{*}{36.53} \bigstrut[t]\\
          & \multicolumn{1}{r|}{} &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-11}          & Hybrid Features & 46.45 & 86.79 & 77.87 & 29.34 & 59.19 & 47.51 & 24.87 & 51.62 & 41.18 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[4]{*}{MIPGAN-II}} & \multirow{2}[2]{*}{Ensemble Features} & \multirow{2}[2]{*}{39.93} & \multirow{2}[2]{*}{73.58} & \multirow{2}[2]{*}{66.89} & \multirow{2}[2]{*}{15.78} & \multirow{2}[2]{*}{28.14} & \multirow{2}[2]{*}{19.38} & \multirow{2}[2]{*}{13.72} & \multirow{2}[2]{*}{28.98} & \multirow{2}[2]{*}{16.63} \bigstrut[t]\\
          & \multicolumn{1}{r|}{} &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-11}          & Hybrid Features & 44.72 & 82.16 & 73.75 & 19.36 & 43.22 & 28.64 & 16.98 & 32.93 & 23.84 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADStyleGAN}%
\end{table}%


%%%% MAD - MIPGAN - I %%%%%%%%


\begin{table}[htbp]
  \centering
  \caption{MAD- MIPGAN-I}
    \begin{tabular}{|c|p{9em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[6]{*}{Morph Generation Type}} & \multirow{3}[6]{*}{MAD Algorithms} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-EER (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER =} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-ERR (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER=} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-EER (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER=} \bigstrut\\
\cline{4-5}\cline{7-8}\cline{10-11}          & \multicolumn{1}{c|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
\cline{3-11}          & \multicolumn{1}{c|}{} & \multicolumn{3}{p{12.705em}|}{Digital} & \multicolumn{3}{p{12.705em}|}{Print-Scan} & \multicolumn{3}{p{12.705em}|}{Print-Scan with Compression} \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Facial Landmarks}} & Ensemble Features & 23.66 & 51.45 & 39.96 & 5.82  & 7.22  & 2.92  & 6.17  & 7.54  & 3.94 \bigstrut\\
\cline{2-11}          & Hybrid Features & 47.15 & 87.16 & 79.41 & 6.5   & 8.23  & 4.15  & 7.91  & 10.29 & 6.34 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 17.72 & 37.33 & 26.58 & 12.19 & 26.24 & 15.26 & 11.82 & 24.69 & 14.23 \bigstrut\\
\cline{2-11}          & Hybrid Features & 31.16 & 64.32 & 53.85 & 11.99 & 19.2  & 13.72 & 9.93  & 18.15 & 9.94 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{2-11}          & Hybrid Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 2.15  & 0.17  & 0     & 0.68  & 0     & 0     & 0.64  & 0     & 0 \bigstrut\\
\cline{2-11}          & Hybrid Features & 1.36  & 0.34  & 0     & 0.86  & 0     & 0     & 0.84  & 0     & 0 \bigstrut\\
    \hline
    \end{tabular}%
  \label{tab:MADMIPGAN-I}%
\end{table}%


%%%% MAD - MIPGAN - II %%%%%%%%


\begin{table}[htbp]
  \centering
  \caption{MAD MIPGAN-II}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|p{10.9em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[6]{*}{Morph Generation Type}} & \multirow{3}[6]{*}{MAD Algorithms} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-EER (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER =} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-ERR (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER=} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{D-EER (\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER@APCER=} \bigstrut\\
\cline{4-5}\cline{7-8}\cline{10-11}          & \multicolumn{1}{c|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
\cline{3-11}          & \multicolumn{1}{c|}{} & \multicolumn{3}{p{12.705em}|}{Digital} & \multicolumn{3}{p{12.705em}|}{Print-Scan} & \multicolumn{3}{p{12.705em}|}{Print-Scan with Compression} \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Facial Landmarks}} & Ensemble Features & 13.08 & 29.15 & 15.78 & 4.28  & 3.94  & 2.22  & 4.28  & 3.61  & 2.22 \bigstrut\\
\cline{2-11}          & Hybrid Features & 40.14 & 77.7  & 67.23 & 5.49  & 5.48  & 2.4   & 7.21  & 10.98 & 4.15 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 12.51 & 22.29 & 15.78 & 13.72 & 29.67 & 18.18 & 14.25 & 31.73 & 2041 \bigstrut\\
\cline{2-11}          & Hybrid Features & 24.7  & 49.74 & 41.85 & 12.87 & 26.58 & 14.75 & 11.86 & 26.92 & 15.09 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 1.56  & 0.68  & 0.34  & 2.14  & 1.22  & 0.53  & 2.57  & 0.85  & 0.34 \bigstrut\\
\cline{2-11}          & Hybrid Features & 2.27  & 0.85  & 0.17  & 4.79  & 4.8   & 3.43  & 4.3   & 3.6   & 2.22 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{2-11}          & Hybrid Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADMIPGAN-II}%
\end{table}%

% Quantitative evaluation of vulnerability of COTS Cognitec-FRS from various morph generation approaches
%vulnerability-report-VGGFace2
\begin{table*}[htbp]
  \centering
    \caption{Quantitative evaluation of vulnerability of VGGFace2\cite{cao2018vggface2} FRS from various morph generation approaches}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \cline{2-7}    \multirow{3}[6]{*}{\textbf{Morph generation type\newline{}\newline{}}} & MMPMR(\%) & FMMPMR(\%) & MMPMR(\%) & FMMPMR(\%) & MMPMR(\%) & FMMPMR(\%) \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{Digital}} & \multicolumn{2}{c|}{\textbf{Print-Scan}} & \multicolumn{2}{c|}{\textbf{Print-Scan with compression}} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{Male} & \multicolumn{2}{c|}{Male} & \multicolumn{2}{c|}{Male} \bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{85.59} & 70.80 & 83.91 & 68.20 & 83.86 & 67.73 \bigstrut\\
    \hline
    Landmark-II & 63.27 & 46.55 & 63.12 & 46.37 & 63.72 & 46.80 \bigstrut\\
    \hline
    StyleGAN & 61.19 & 41.01 & 61.68 & 41.43 & 61.68 & 41.04 \bigstrut\\
    \hline
    MIPGAN-I & 76.96 & 59.24 & 76.96 & 57.16 & 76.07 & 57.31 \bigstrut\\
    \hline
    MIPGAN-II & 75.73 & 56.97 & 72.87 & 54.57 & 72.87 & 54.43 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{Female} & \multicolumn{2}{c|}{Female} & \multicolumn{2}{c|}{Female} \bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{96.03} & 83.55 & 93.95 & 82.02 & 93.32 & 81.39 \bigstrut\\
    \hline
    Landmark-II & 87.76 & 71.85 & 89.39 & 73.82 & 89.80 & 74.27 \bigstrut\\
    \hline
    StyleGAN & 80.42 & 59.19 & 79.79 & 59.10 & 78.54 & 58.83 \bigstrut\\
    \hline
    MIPGAN-I & 90.41 & 76.68 & 89.39 & 75.95 & 89.18 & 75.85 \bigstrut\\
    \hline
    MIPGAN-II & 88.98 & 75.42 & 87.96 & 74.54 & 88.37 & 74.90 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{Combined} & \multicolumn{2}{c|}{Combined} & \multicolumn{2}{c|}{Combined}\bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{87.64} & 72.82 & 85.87 & 70.39 & 85.71 & 69.90 \bigstrut\\
    \hline
    Landmark-II & 68.07 & 50.64 & 68.27 & 50.80 & 68.86 & 51.28 \bigstrut\\
    \hline
    StyleGAN & 64.92 & 43.91 & 65.20 & 44.25 & 64.96 & 43.88 \bigstrut\\
    \hline
    MIPGAN-I & 79.61 & 62.06 & 79.41 & 60.19 & 78.66 & 60.30 \bigstrut\\
    \hline
    MIPGAN-II & 78.34 & 59.95 & 75.84 & 57.80 & 75.92 & 57.73 \bigstrut\\
    \hline

    \end{tabular}%
    }
  \label{tab:vulnerability-report-VGGFace2}%
\end{table*}%

%vulnerability-report-Arcface
\begin{table*}[htbp]
  \centering
    \caption{Quantitative evaluation of vulnerability of Arcface\cite{deng2019arcface} FRS from various morph generation approaches}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \cline{2-7}    \multirow{3}[6]{*}{\textbf{Morph generation type\newline{}\newline{}}} & MMPMR(\%) & FMMPMR(\%) & MMPMR(\%) & FMMPMR(\%) & MMPMR(\%) & FMMPMR(\%) \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{Digital}} & \multicolumn{2}{c|}{\textbf{Print-Scan}} & \multicolumn{2}{c|}{\textbf{Print-Scan with compression}} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{Male} & \multicolumn{2}{c|}{Male} & \multicolumn{2}{c|}{Male} \bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{99.60} & 98.19 & 97.38 & 96.88 & 97.33 & 96.70 \bigstrut\\
    \hline
    Landmark-II & 91.09 & 84.62 & 93.45 & 86.42 & 93.60 & 86.02 \bigstrut\\
    \hline
    StyleGAN & 70.99 & 55.76 & 73.86 & 58.67 & 73.32 & 58.26 \bigstrut\\
    \hline
    MIPGAN-I & 93.70 & 85.17 & 92.76 & 84.39 & 93.01 & 84.41 \bigstrut\\
    \hline
    MIPGAN-II & 93.65 & 86.45 & 93.55 & 85.30 & 93.25 & 85.06 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{Female} & \multicolumn{2}{c|}{Female} & \multicolumn{2}{c|}{Female} \bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{99.79} & 97.01 & 99.79 & 96.91 & 99.79 & 97.01 \bigstrut\\
    \hline
    Landmark-II & 94.49 & 86.71 & 97.76 & 89.76 & 98.16 & 89.17 \bigstrut\\
    \hline
    StyleGAN & 80.21 & 63.22 & 82.71 & 65.70 & 82.71 & 66.05 \bigstrut\\
    \hline
    MIPGAN-I & 97.35 & 89.53 & 97.96 & 91.02 & 97.76 & 91.02 \bigstrut\\
    \hline
    MIPGAN-II & 96.33 & 89.47 & 95.92 & 89.33 & 96.12 & 89.42 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{Combined} & \multicolumn{2}{c|}{Combined} & \multicolumn{2}{c|}{Combined}\bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{99.68} & 98.00 & 97.88 & 96.89 & 97.84 & 96.75 \bigstrut\\
    \hline
    Landmark-II & 91.79 & 84.96 & 94.33 & 86.96 & 94.53 & 86.54 \bigstrut\\
    \hline
    StyleGAN & 72.80 & 56.95 & 75.60 & 59.79 & 75.16 & 59.51 \bigstrut\\
    \hline
    MIPGAN-I & 94.45 & 85.94 & 93.81 & 85.46 & 93.97 & 85.48 \bigstrut\\
    \hline
    MIPGAN-II & 94.21 & 86.94 & 94.05 & 85.95 & 93.85 & 85.77 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:vulnerability-report-Arcface}%
\end{table*}%

%vulnerability-report-LCNN29
\begin{table*}[htbp]
  \centering
    \caption{Quantitative evaluation of vulnerability of LCNN-29\cite{wu2018light} FRS from various morph generation approaches}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \cline{2-7}    \multirow{3}[6]{*}{\textbf{Morph generation type\newline{}\newline{}}} & MMPMR(\%) & FMMPMR(\%) & MMPMR(\%) & FMMPMR(\%) & MMPMR(\%) & FMMPMR(\%) \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{Digital}} & \multicolumn{2}{c|}{\textbf{Print-Scan}} & \multicolumn{2}{c|}{\textbf{Print-Scan with compression}} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{Male} & \multicolumn{2}{c|}{Male} & \multicolumn{2}{c|}{Male} \bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{96.63} & 89.28 & 95.25 & 89.36 & 94.80 & 88.62 \bigstrut\\
    \hline
    Landmark-II & 75.09 & 60.72 & 74.64 & 57.81 & 82.43 & 68.32 \bigstrut\\
    \hline
    StyleGAN & 83.12 & 66.44 & 85.20 & 69.54 & 84.85 & 68.88 \bigstrut\\
    \hline
    MIPGAN-I & 95.13 & 86.35 & 94.04 & 84.39 & 94.09 & 84.30 \bigstrut\\
    \hline
    MIPGAN-II & 94.93 & 85.14 & 93.94 & 83.14 & 93.75 & 82.63 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{Female} & \multicolumn{2}{c|}{Female} & \multicolumn{2}{c|}{Female} \bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{99.16} & 95.00 & 98.75 & 94.26 & 98.96 & 94.49 \bigstrut\\
    \hline
    Landmark-II & 92.04 & 82.28 & 94.69 & 82.85 & 95.92 & 86.98 \bigstrut\\
    \hline
    StyleGAN & 93.33 & 80.08 & 92.92 & 83.06 & 92.92 & 82.76 \bigstrut\\
    \hline
    MIPGAN-I & 97.76 & 92.27 & 96.94 & 91.59 & 96.94 & 91.44 \bigstrut\\
    \hline
    MIPGAN-II & 95.71 & 90.72 & 95.31 & 89.85 & 95.71 & 89.58 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{Combined} & \multicolumn{2}{c|}{Combined} & \multicolumn{2}{c|}{Combined}\bigstrut\\
    \hline
    Landmark-I & \multicolumn{1}{c|}{97.16} & 90.19 & 95.96 & 90.14 & 95.64 & 89.55 \bigstrut\\
    \hline
    Landmark-II & 78.42 & 64.20 & 78.58 & 61.85 & 85.11 & 71.36 \bigstrut\\
    \hline
    StyleGAN & 85.12 & 68.61 & 86.72 & 71.69 & 86.44 & 71.09 \bigstrut\\
    \hline
    MIPGAN-I & 95.68 & 87.30 & 94.64 & 85.55 & 94.68 & 85.45 \bigstrut\\
    \hline
    MIPGAN-II & 95.12 & 86.05 & 94.25 & 84.23 & 94.17 & 83.75 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:vulnerability-report-LCNN29}%
\end{table*}%



%%%% updated PSNR and SSIM %%%%%%%%
\begin{table}[htbp]
  \centering
  \caption{Quality analysis using PSNR and SSIM}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|p{11.435em}|l|l|}
    \hline
    \textbf{Morph generation Methods} & \multicolumn{1}{p{3.165em}|}{\textbf{PSNR}} & \multicolumn{1}{p{3.2em}|}{\textbf{SSIM}} \bigstrut\\
    \hline
    Landmark-I   & 21.111 & 0.761 \bigstrut\\
    \hline
    Landmark-II   & 20.274 & 0.736 \bigstrut\\
    \hline
    StyleGAN & 20.135 & 0.720 \bigstrut\\
    \hline
    MIPGAN-I & 21.013 & 0.757 \bigstrut\\
    \hline
    MIPGAN-II & 20.831 & 0.759 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:PSNRnSSIM}%
\end{table}%


%%%%% Updated ablation vulnerability table

\begin{table}[htbp]
  \centering
  \caption{Vulnerability results of ablation study}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|p{5.4em}|p{6.135em}|p{6.4em}|p{6.765em}|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{3}[6]{*}{\textbf{Final ID}} & \multirow{3}[6]{*}{\textbf{Identity loss}} & \multirow{3}[6]{*}{\textbf{MSSIM}} & \multirow{3}[6]{*}{\textbf{Perceptual}} & \multicolumn{4}{p{16.94em}|}{\textbf{MIPGAN-I}} & \multicolumn{4}{p{16.94em}|}{\textbf{MIPGAN-II}} \bigstrut\\
\cline{5-12}    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{p{8.47em}|}{FMMPMR} & \multicolumn{2}{p{8.47em}|}{MMPMR} & \multicolumn{2}{p{8.47em}|}{FMMPMR} & \multicolumn{2}{p{8.47em}|}{MMPMR} \bigstrut\\
\cline{5-12}    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{4.235em}|}{Cognitec} & \multicolumn{1}{p{4.235em}|}{ArcFace} & \multicolumn{1}{p{4.235em}|}{Cognitec} & \multicolumn{1}{p{4.235em}|}{ArcFace} & \multicolumn{1}{p{4.235em}|}{Cognitec} & \multicolumn{1}{p{4.235em}|}{ArcFace} & \multicolumn{1}{p{4.235em}|}{Cognitec} & \multicolumn{1}{p{4.235em}|}{ArcFace} \bigstrut\\
    \hline
    Final ID & -     & -     & -     & 81.82 & 75.87 & 90.69 & 93.4  & 77.83 & 71.98 & 90.1  & 91.18 \bigstrut\\
    \hline
    -     & Identity loss & -     & -     & 78    & 62.15 & 89.17 & 83.77 & 78.39 & 64.51 & 90.04 & 82.54 \bigstrut\\
    \hline
    -     & -     & MSSIM & -     & 80.82 & 73.33 & 91.81 & 92.66 & 78.73 & 71.79 & 89.58 & 90.55 \bigstrut\\
    \hline
    -     & -     & -     & Perceptual & 21.37 & 47.85 & 44.1  & 71.95 & 11.92 & 33.12 & 29.47 & 59.5 \bigstrut\\
    \hline
    -     & -     & -     & -     & \textbf{84.65} & \textbf{85.94} & \textbf{94.36} & \textbf{94.45} & \textbf{81.59} & \textbf{86.24} & \textbf{92.93} & \textbf{94.21} \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:vulablation}%
\end{table}%


%%%%%%%% Hyper parameters results %%%%%%%


\begin{table}[htbp]
  \centering
  \caption{Quantitative results of hyper-parameters study}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|p{5.8em}|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{2}[4]{*}{Proposed Morph Generators}} & \multirow{2}[4]{*}{Case-study} & \multicolumn{4}{p{16.94em}|}{Hyper-parameters} & \multicolumn{2}{p{8.47em}|}{MMPMR (\%)} & \multicolumn{2}{p{8.47em}|}{FMMPMR (\%)} \bigstrut\\
\cline{3-10}          & \multicolumn{1}{r|}{} & 1     & 2     & 3     & 4     & \multicolumn{1}{p{4.235em}|}{Cognitec} & \multicolumn{1}{p{4.235em}|}{ArcFace} & \multicolumn{1}{p{4.235em}|}{Cognitec} & \multicolumn{1}{p{4.235em}|}{ArcFace} \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{5}[10]{*}{MIPGAN -I}} & C-1   & 0.0004 & 10    & 1     & 1     & 93.94 & 93.49 & 84.39 & 75.61 \bigstrut\\
\cline{2-10}          & C-2   & 0.0001 & 10    & 1     & 1     & 92.66 & 91.15 & 79.66 & 72.94 \bigstrut\\
\cline{2-10}          & C-3   & 0.0002 & 1     & 10    & 1     & 94.17 & 91.9  & 84.34 & 75.66 \bigstrut\\
\cline{2-10}          & C-4   & 0.0002 & 1     & 1     & 10    & 83.16 & 82.14 & 67.19 & 59.46 \bigstrut\\
\cline{2-10}          & Proposed & 0.0002 & 10    & 1     & 1     & 94.36 & 94.45 & 84.65 & 85.94 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{5}[10]{*}{MIPGAN -II}} & C-1   & 0.0004 & 10    & 1     & 1     & 91.36 & 91.98 & 81.29 & 76.18 \bigstrut\\
\cline{2-10}          & C-2   & 0.0001 & 10    & 1     & 1     & 91.69 & 88.29 & 73.91 & 68.16 \bigstrut\\
\cline{2-10}          & C-3   & 0.0002 & 1     & 10    & 1     & 90.63 & 90.91 & 80.76 & 75.87 \bigstrut\\
\cline{2-10}          & C-4   & 0.0002 & 1     & 1     & 10    & 87.22 & 74.33 & 57.43 & 51.91 \bigstrut\\
\cline{2-10}          & Proposed & 0.0002 & 10    & 1     & 1     & 92.93 & 94.21 & 81.59 & 86.94 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:hyperparameterRes}%
\end{table}%







% on the digital version of the morphed face images. 
%% Vulnerability (MMPMR and FMMPMR) - Ablation study
%%%\begin{table*}[htbp]
  %\centering
 % \caption{Vulnerability - Ablation study on the proposed loss function}
 % \resizebox{1\linewidth}{!}{
   % \begin{tabular}{|p{5.765em}|p{5.435em}|p{7.335em}|p{6.9em}|r|r|r|r|}
   % \hline
   % \multirow{2}[4]{*}{\textbf{$Loss_{ID-Diff}$}} & \multirow{2}[4]{*}{\textbf{$Loss_{Identity}$}} & %\multirow{2}[4]{*}{\textbf{$Loss_{MS-SSIM}$}} & \multirow{2}[4]{*}{\textbf{$Loss_{Perceptual}$}} & %\multicolumn{2}{p{11.2em}|}{\textbf{MIPGAN-I}} & \multicolumn{2}{p{12.77em}|}{\textbf{MIPGAN-II}} \bigstrut\\
%\cline{5-8}    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{p{5.535em}|}{FMMPMR (\%)} & \multicolumn{1}{p{5.665em}|}{MMPMR (\%)} & \multicolumn{1}{p{5.635em}|}{FMMPMR (\%)} & \multicolumn{1}{p{7.135em}|}{MMPMR (\%)} \bigstrut\\
   % \hline
  %  \ding{53} & \ding{51}    & \ding{51}     & \ding{51}    & 81.82 & 90.69 & 77.83 & 90.12 \bigstrut\\
  %  \hline
   %\ding{51}     & \ding{53} & \ding{51}     & \ding{51}     & 78.15 & 89.17 & 78.39 & 90.04 \bigstrut\\
    %\hline
   % \ding{51}     & \ding{51}    & \ding{53} & \ding{51}     & 80.82 & 91.81 & 78.73 & 89.58 \bigstrut\\
   % \hline
  %  \ding{51}     & \ding{51}    & \ding{51}     & \ding{53} & 21.37 & 44.18 & 11.92 & 29.47 \bigstrut\\
   % \hline
   % \ding{51}    & \ding{51}     & \ding{51}     & \ding{51}     & \textbf{84.65} & \textbf{94.36} & \textbf{81.59} & %\textbf{92.93} \bigstrut\\
  %  \hline
   % \end{tabular}%
  %  }
  %\label{tab:Abalation}%
%\end{table*}%




%%%%% UPdated MAD table (training and testing)%%%%%%%%


% Table generated by Excel2LaTeX from sheet 'Sheet10'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{MAD Algorithms}}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       &       & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       &       &       &       &       &       &       &       &       &       &  \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{20}[20]{*}{\textbf{Landmarks-I}}} & \multicolumn{1}{r|}{\multirow{4}[4]{*}{Landmarks-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          &       & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{4}[4]{*}{Landmarks-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          &       & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{4}[4]{*}{StyleGAN}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          &       & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{4}[4]{*}{MIPGAN-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          &       & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{4}[4]{*}{MIPGAN-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          &       & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
    \hline
    \multicolumn{1}{|c|}{\multirow{20}[20]{*}{\textbf{Landmarks-II}}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{StyleGAN}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
    \hline
    \multicolumn{1}{|c|}{\multirow{20}[20]{*}{\textbf{StyleGAN}}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{StyleGAN}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
    \hline
    \multicolumn{1}{|c|}{\multirow{20}[20]{*}{\textbf{MIPGAN-I}}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{StyleGAN}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
    \hline
    \multicolumn{1}{|c|}{\multirow{20}[20]{*}{\textbf{MIPGAN-II}}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Landmarks-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{4}[4]{*}{Landmarks-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          &       & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{StyleGAN}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-I}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{MIPGAN-II}} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Hybrid Features }} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
\cline{3-12}          & \multirow{2}[2]{*}{} & \multicolumn{1}{r|}{\multirow{2}[2]{*}{Ensemble Features}} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} & \multirow{2}[2]{*}{} \bigstrut[t]\\
          &       &       &       &       &       &       &       &       &       &       &  \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%





%%%%%%%%%% MAD table revised (Train:Landmarks-I) %%%%%%%%%%


\begin{table}[htbp]
  \centering
  \caption{Quantitative performance of MAD - Training- Landmarks-I}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|r|r|p{6.565em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       & \multicolumn{1}{r|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{\multirow{10}[20]{*}{\textbf{Landmarks-I}}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-I}} & Ensemble Features & 0     & 0     & 0     & 2.35  & 1.45  & 0.96  & 2.58  & 1.71  & 1.54 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 0.16  & 0     & 0     & 1.85  & 0.85  & 0.34  & 2.25  & 1.12  & 0.51 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-II}} & Ensemble Features & 49.55 & 92.22 & 88.85 & 41.93 & 81.45 & 76.25 & 42.15 & 83.88 & 77.64 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 49.16 & 99.31 & 97.59 & 44.17 & 86.48 & 80.24 & 46.49 & 88.38 & 81.95 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 0.22  & 0     & 0     & 13.36 & 27.44 & 16.46 & 14.77 & 27.27 & 19.38 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 0.16  & 0     & 0     & 44.96 & 83.7  & 75.47 & 9.44  & 14.57 & 9.14 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 39.16 & 73.14 & 65.35 & 9.45  & 14.57 & 8.74  & 8.95  & 15.26 & 9.26 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 46.82 & 86.62 & 81.64 & 12.32 & 19.72 & 13.2  & 9.74  & 15.95 & 8.91 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 34.13 & 70.49 & 61.57 & 5.32  & 6.68  & 2.57  & 6.72  & 8.16  & 4.14 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 44.96 & 83.7  & 75.47 & 5.9   & 8.42  & 3.23  & 5.67  & 6.18  & 2.91 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADlandmark1}%
\end{table}%

%%%%%%%%%%% MAD table revised (Train: Landmarks-II) %%%%

% Table generated by Excel2LaTeX from sheet 'Sheet15'
\begin{table}[htbp]
  \centering
  \caption{Quantitative performance of MAD - Training- Landmarks-II}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|r|p{7.6em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       & \multicolumn{1}{r|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{10}[20]{*}{\textbf{Landmarks-II}}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-I}} & Ensemble Features & 48.57 & 97.77 & 95.36 & 24.19 & 52.48 & 43.22 & 21.64 & 47.51 & 36.19 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 45.67 & 96.91 & 94.16 & 32.26 & 77.87 & 66.55 & 24.51 & 50.94 & 40.65 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-II}} & Ensemble Features & 3.62  & 2.22  & 0.68  & 6.32  & 7.97  & 2.42  & 5.57  & 6.41  & 2.42 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 1.53  & 0.17  & 0     & 5.21  & 5.19  & 3.14  & 5.37  & 5.71  & 3.46 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 29.67 & 61.92 & 52.48 & 27.18 & 61.57 & 50.6  & 29.18 & 62.14 & 52.48 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 34.76 & 74.44 & 62.95 & 34.8  & 67.23 & 58.14 & 23.17 & 49.22 & 38.25 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 30.23 & 65.35 & 53.17 & 43.92 & 87.65 & 79.24 & 44.24 & 89.23 & 82.33 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 46.29 & 84.04 & 77.01 & 34.16 & 71.18 & 64.66 & 35.5  & 76.84 & 65.52 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 27.13 & 58.83 & 45.45 & 33.57 & 77.35 & 65.52 & 40.46 & 84.9  & 75.47 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 46.82 & 83.53 & 75.81 & 35.91 & 77.18 & 65.24 & 36.5  & 79.24 & 68.78 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADlandmark2}%
\end{table}%




%%%%%%%%%% MAD table revised (Train: StyleGAN) 

\begin{table}[htbp]
  \centering
  \caption{Quantitative performance of MAD - Training- StyleGAN}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|r|p{7.035em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       & \multicolumn{1}{r|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{10}[20]{*}{\textbf{StyleGAN}}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-I}} & Ensemble Features & 0.32  & 0     & 0     & 16.6  & 28.13 & 19.89 & 13.89 & 22.12 & 17.66 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 0.42  & 0     & 0     & 15.26 & 26.41 & 17.66 & 14.37 & 22.81 & 16.92 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-II}} & Ensemble Features & 44.72 & 89.53 & 80.61 & 38.31 & 78.5  & 69.15 & 38.84 & 83.7  & 74.17 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 45.65 & 90.22 & 84.56 & 34.18 & 81.95 & 70.53 & 32.93 & 78.5  & 64.12 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 39.97 & 75.98 & 68.78 & 20.21 & 42.14 & 33.44 & 20.73 & 45.28 & 36.53 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 46.45 & 86.79 & 77.87 & 29.34 & 59.19 & 47.51 & 24.87 & 51.62 & 41.18 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 39.93 & 73.58 & 66.89 & 15.78 & 28.14 & 19.38 & 13.72 & 28.98 & 16.63 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 44.72 & 82.16 & 73.75 & 19.36 & 43.22 & 28.64 & 16.98 & 32.93 & 23.84 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADstylegan}%
\end{table}%


%%%%%%%%%% MAD table revised (Train: MIPGAN-I) 

\begin{table}[htbp]
  \centering
  \caption{Quantitative performance of MAD - Training- MIPGAN-I}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|r|p{9.8em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       & \multicolumn{1}{r|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{10}[20]{*}{\textbf{MIPGAN-I}}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-I}} & Ensemble Features & 23.66 & 51.45 & 39.96 & 5.82  & 7.22  & 2.92  & 6.17  & 7.54  & 3.94 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 47.15 & 87.16 & 79.41 & 6.5   & 8.23  & 4.15  & 7.91  & 10.29 & 6.34 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-II}} & Ensemble Features & 35.38 & 82.33 & 68.95 & 41.67 & 95.14 & 83.53 & 43.68 & 96.01 & 85.44 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 28.62 & 75.64 & 61.4  & 44.38 & 95.66 & 85.78 & 38.18 & 90.46 & 78.16 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 17.72 & 37.22 & 26.58 & 12.19 & 26.24 & 15.26 & 11.82 & 24.69 & 14.23 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 31.16 & 64.32 & 53.85 & 11.99 & 19.2  & 13.72 & 9.93  & 18.15 & 9.94 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 2.15  & 0.17  & 0     & 0.68  & 0     & 0     & 0.64  & 0     & 0 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 1.36  & 0.34  & 0     & 0.86  & 0     & 0     & 0.8461 & 0     & 0 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADMIPGAN1}%
\end{table}%


%%%%%%%%%% MAD table revised (Train: MIPGAN-II)

\begin{table}[htbp]
  \centering
  \caption{Quantitative performance of MAD - Training- MIPGAN-II}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|r|p{7.435em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       & \multicolumn{1}{r|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{10}[20]{*}{\textbf{MIPGAN-II}}} & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-I}} & Ensemble Features & 13.08 & 29.15 & 15.78 & 4.28  & 3.94  & 2.22  & 4.28  & 3.61  & 2.22 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 40.14 & 77.7  & 67.23 & 5.49  & 5.48  & 2.4   & 7.21  & 10.98 & 4.15 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{Landmarks-II}} & Ensemble Features & 32.37 & 84.9  & 70.32 & 39.2  & 90.12 & 82.32 & 44.17 & 95.49 & 88.73 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 23.88 & 63.8  & 45.62 & 40.22 & 88.9  & 79.2  & 38.96 & 94.28 & 82.14 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{StyleGAN}} & Ensemble Features & 12.51 & 22.29 & 15.78 & 13.72 & 29.67 & 18.18 & 14.25 & 31.73 & 20.41 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 24.7  & 49.74 & 41.85 & 12.87 & 26.58 & 14.75 & 11.86 & 26.92 & 15.09 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features & 1.56  & 0.68  & 0.34  & 2.14  & 1.22  & 0.53  & 2.57  & 0.85  & 0.34 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 2.27  & 0.85  & 0.17  & 4.79  & 4.8   & 3.43  & 4.3   & 3.6   & 2.22 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{r|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{3-12}          &       & Hybrid Features & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADMIPGAN2}%
\end{table}%

%%%%%%%%%%%%%%%%%%%% vulnerability revised

%%%%%%%%% Neurotec Vulnerability %%%%%%%%
\begin{table}[htbp]
  \centering
  \caption{Quantitative evaluation of vulnerability of COTS Neurotec FRS from various morph generation approaches}
    \begin{tabular}{|p{8.4em}|c|c|c|c|c|c|}
    \hline
    \multirow{3}[6]{*}{\textbf{Morph Generation Type}} & \multicolumn{1}{p{5.6em}|}{MMPMR(\%)} & \multicolumn{1}{p{5.8em}|}{FMMPMR(\%)} & \multicolumn{1}{p{5.335em}|}{MMPMR(\%)} & \multicolumn{1}{p{5.465em}|}{FMMPMR(\%)} & \multicolumn{1}{p{5.665em}|}{MMPMR(\%)} & \multicolumn{1}{p{6.3em}|}{FMMPMR(\%)} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{p{11.4em}|}{\textbf{Digital}} & \multicolumn{2}{p{10.8em}|}{\textbf{Print-Scan}} & \multicolumn{2}{p{11.965em}|}{\textbf{Print-Scan with Compression}} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{p{11.4em}|}{Male} & \multicolumn{2}{p{10.8em}|}{Male} & \multicolumn{2}{p{11.965em}|}{Male} \bigstrut\\
    \hline
    Landmark-I & 99.4  & 94.7  & 95.45 & 83.71 & 93.23 & 77.16 \bigstrut\\
    \hline
    Landmark-II & 88.99 & 68.51 & 88.92 & 63.31 & 80.62 & 53.63 \bigstrut\\
    \hline
    StyleGAN & 52.26 & 26.47 & 31.88 & 12.98 & 31.6  & 12.15 \bigstrut\\
    \hline
    MIPGAN-I & 58.18 & 32.56 & 32.59 & 25.33 & 57.6  & 53.52 \bigstrut\\
    \hline
    MIPGAN-II & 53.16 & 29.65 & 47.41 & 20.71 & 50.73 & 23.72 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{2}{p{11.4em}|}{Female} & \multicolumn{2}{p{10.8em}|}{Female} & \multicolumn{2}{p{11.965em}|}{Female} \bigstrut\\
    \hline
    Landmark-I & 100   & 99.25 & 100   & 98.11 & 98.74 & 91.18 \bigstrut\\
    \hline
    Landmark-II & 94.69 & 85.96 & 97.49 & 84.92 & 95.4  & 78.89 \bigstrut\\
    \hline
    StyleGAN & 70.6  & 50.13 & 55.2  & 25.72 & 52.39 & 26.19 \bigstrut\\
    \hline
    MIPGAN-I & 80.98 & 56.29 & 73.06 & 46.87 & 77.89 & 30.5 \bigstrut\\
    \hline
    MIPGAN-II & 74.79 & 49.45 & 69.59 & 42.17 & 70.73 & 46.18 \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{2}{p{11.4em}|}{Combined} & \multicolumn{2}{p{10.8em}|}{Combined} & \multicolumn{2}{p{11.965em}|}{Combined} \bigstrut\\
    \hline
    Landmark-I & 99.51 & 95.37 & 96.32 & 85.43 & 94.3  & 79.25 \bigstrut\\
    \hline
    Landmark-II & 90.16 & 71.17 & 90.59 & 66.67 & 83.5  & 57.38 \bigstrut\\
    \hline
    StyleGAN & 55.06 & 29.39 & 36.36 & 14.83 & 35.62 & 14.28 \bigstrut\\
    \hline
    MIPGAN-I & 63.22 & 35.73 & 40.46 & 28.71 & 61.66 & 34.14 \bigstrut\\
    \hline
    MIPGAN-II & 57.47 & 31.45 & 51.72 & 23.54 & 54.94 & 27.46 \bigstrut\\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%



%%%%%

% Table generated by Excel2LaTeX from sheet 'Sheet17'
\begin{table}[htbp]
  \centering
  \caption{Quantitative evaluation of vulnerability of COTS Cognitec-FRS from various morph generation approaches}
   \resizebox{1\linewidth}{!}{
    \begin{tabular}{|p{6.8em}|c|c|c|c|c|c|}
    \hline
    \multirow{3}[6]{*}{\textbf{Morph Generation Type}} & \multicolumn{1}{p{6.335em}|}{MMPMR(\%)} & \multicolumn{1}{p{6.965em}|}{FMMPMR(\%)} & \multicolumn{1}{p{7.5em}|}{MMPMR(\%)} & \multicolumn{1}{p{7.135em}|}{FMMPMR(\%)} & \multicolumn{1}{p{7.265em}|}{MMPMR(\%)} & \multicolumn{1}{p{7.465em}|}{FMMPMR(\%)} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{p{13.3em}|}{\textbf{Digital}} & \multicolumn{2}{p{14.635em}|}{\textbf{Print-Scan}} & \multicolumn{2}{p{14.73em}|}{\textbf{Print-Scan with Compression}} \bigstrut\\
\cline{2-7}    \multicolumn{1}{|c|}{} & \multicolumn{2}{p{13.3em}|}{Male} & \multicolumn{2}{p{14.635em}|}{Male} & \multicolumn{2}{p{14.73em}|}{Male} \bigstrut\\
    \hline
    Landmark-I \cite{raghavendra2017face} & 100   & 98.77 & 97.23 & 97.34 & 97.38 & 96.95 \bigstrut\\
    \hline
    Landmark-II \cite{UBO_Morphing_Tool} & 87.29 & 76.86 & 90.32 & 78.23 & 88.78 & 77.14 \bigstrut\\
    \hline
    StyleGAN \cite{MorphStyleGAN2020} & 63.51 & 41.27 & 60.59 & 39.51 & 57.12 & 35.05 \bigstrut\\
    \hline
    MIPGAN-I & 93.35 & 83.08 & 91.72 & 80.55 & 91.07 & 77.89 \bigstrut\\
    \hline
    MIPGAN-II & 92.22 & 80.45 & 90.74 & 77.67 & 89.16 & 73.47 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{p{13.3em}|}{Female} & \multicolumn{2}{p{14.635em}|}{Female} & \multicolumn{2}{p{14.73em}|}{Female} \bigstrut\\
    \hline
    Landmark-I \cite{raghavendra2017face} & 100   & 99.26 & 99.37 & 99.02 & 99.78 & 99.24 \bigstrut\\
    \hline
    Landmark-II \cite{UBO_Morphing_Tool} & 94.28 & 88.67 & 98.22 & 91.48 & 98.16 & 90.97 \bigstrut\\
    \hline
    StyleGAN \cite{MorphStyleGAN2020} & 68.75 & 42.62 & 66.45 & 42.01 & 66.45 & 40.49 \bigstrut\\
    \hline
    MIPGAN-I & 98.57 & 93.11 & 98.16 & 91.22 & 96.12 & 90.52 \bigstrut\\
    \hline
    MIPGAN-II & 95.91 & 87.66 & 95.3  & 86.26 & 94.69 & 84.47 \bigstrut\\
    \hline
    \multicolumn{1}{|r|}{} & \multicolumn{2}{p{13.3em}|}{Combined} & \multicolumn{2}{p{14.635em}|}{Combined} & \multicolumn{2}{p{14.73em}|}{Combined} \bigstrut\\
    \hline
    Landmark-I \cite{raghavendra2017face} & 100   & 98.84 & 97.64 & 97.6  & 97.84 & 97.3 \bigstrut\\
    \hline
    Landmark-II \cite{UBO_Morphing_Tool} & 88.65 & 78.72 & 91.85 & 81.56 & 90.61 & 79.33 \bigstrut\\
    \hline
    StyleGAN \cite{MorphStyleGAN2020} & 64.68 & 41.49 & 61.72 & 39.9  & 58.92 & 35.89 \bigstrut\\
    \hline
    MIPGAN-I & 94.36 & 84.65 & \multicolumn{1}{p{7.5em}|}{92.97  } & 82.23 & 92.29 & 79.88 \bigstrut\\
    \hline
    MIPGAN-II & 92.93 & 81.59 & 80.56 & 79.02 & 90.24 & 75.2 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:vulnerability-report}%
\end{table}%


%%%%%%%%%FaceForensics++MAD############
\begin{table*}[htbp]
  \centering
  \caption{Quantitative performance of MAD - Training- MIPGAN-II}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|p{10.435em}|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Training}}} & \multicolumn{1}{r|}{\multirow{3}[6]{*}{\textbf{Morph Generation Type: Testing}}} & \multirow{3}[6]{*}{\textbf{MAD Algorithms}} & \multicolumn{3}{p{12.705em}|}{\textbf{Digital}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan}} & \multicolumn{3}{p{12.705em}|}{\textbf{Print-scan with compression}} \bigstrut\\
\cline{4-12}          &       & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } & \multicolumn{1}{c|}{\multirow{2}[4]{*}{D-EER(\%)}} & \multicolumn{2}{p{8.47em}|}{BPCER @ APCER =  } \bigstrut\\
\cline{5-6}\cline{8-9}\cline{11-12}          &       & \multicolumn{1}{r|}{} &       & 5\%   & 10\%  &       & 5\%   & 10\%  &       & 5\%   & 10\% \bigstrut\\
    \hline
    \multicolumn{1}{|c|}{\multirow{10}[20]{*}{\textbf{MIPGAN-II}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{Landmarks-I \cite{raghavendra2017face}}} & Ensemble Features \cite{EnsembleFeatures_2020} & 13.08 & 29.15 & 15.78 & 4.28  & 3.94  & 2.22  & 4.28  & 3.61  & 2.22 \bigstrut\\
\cline{3-12}          &       & Hybrid Features \cite{RagISBA2019} & 40.14 & 77.7  & 67.23 & 5.49  & 5.48  & 2.4   & 7.21  & 10.98 & 4.15 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{c|}{\multirow{2}[4]{*}{Landmarks-II \cite{UBO_Morphing_Tool}}} & Ensemble Features \cite{EnsembleFeatures_2020} & 32.37 & 84.9  & 70.32 & 39.2  & 90.12 & 82.32 & 44.17 & 95.49 & 88.73 \bigstrut\\
\cline{3-12}          &       & Hybrid Features \cite{RagISBA2019} & 23.88 & 63.8  & 45.62 & 40.22 & 88.9  & 79.2  & 38.96 & 94.28 & 82.14 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{c|}{\multirow{2}[4]{*}{StyleGAN \cite{MorphStyleGAN2020}}} & Ensemble Features \cite{EnsembleFeatures_2020} & 12.51 & 22.29 & 15.78 & 13.72 & 29.67 & 18.18 & 14.25 & 31.73 & 20.41 \bigstrut\\
\cline{3-12}          &       & Hybrid Features \cite{RagISBA2019} & 24.7  & 49.74 & 41.85 & 12.87 & 26.58 & 14.75 & 11.86 & 26.92 & 15.09 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{c|}{\multirow{2}[4]{*}{MIPGAN-I}} & Ensemble Features \cite{EnsembleFeatures_2020} & 1.56  & 0.68  & 0.34  & 2.14  & 1.22  & 0.53  & 2.57  & 0.85  & 0.34 \bigstrut\\
\cline{3-12}          &       & Hybrid Features \cite{RagISBA2019} & 2.27  & 0.85  & 0.17  & 4.79  & 4.8   & 3.43  & 4.3   & 3.6   & 2.22 \bigstrut\\
\cline{2-12}          & \multicolumn{1}{c|}{\multirow{2}[4]{*}{MIPGAN-II}} & Ensemble Features \cite{EnsembleFeatures_2020} & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
\cline{3-12}          &       & Hybrid Features \cite{RagISBA2019} & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:MADMIPGAN2}%
\end{table*}%



